Deep Manifold Prior

We present a prior for manifold structured data, such as surfaces of 3D shapes, where deep neural networks are adopted to reconstruct a target shape using gradient descent starting from a random initialization. We show that surfaces generated this way are smooth, with limiting behavior characterized by Gaussian processes, and we mathematically derive such properties for fully-connected as well as convolutional networks. We demonstrate our method in a variety of manifold reconstruction applications, such as point cloud denoising and interpolation, achieving considerably better results against competitive baselines while requiring no training data. We also show that when training data is available, our method allows developing alternate parametrizations of surfaces under the framework of AtlasNet, leading to a compact network architecture and better reconstruction results on standard image to shape reconstruction benchmarks.

==> experiments2.tex <==
\section{Experiments}
\label{sec:experiments}


\begin{figure}[t]
\centering
\includegraphics[width=0.8\linewidth]{imgs/comp.pdf}
	\caption{\label{fig:comp} \small
	\textbf{Comparison between different convolutional generators.} \small
	We compare image-to-shape reconstruction results using MRTNet~\cite{mrt18} (1D convolutional network) vs. our method (2D convolutional network) using a single decoder and multiple (32) decoders respectively.
	MRTNet generates 4K points whereas the single decoder and 32 decoder models generate 16K and 32K, respectively. Compared to our single decoder output, MRTNet generates surfaces that are less smooth but it's able to capture thin structures and holes such as around the chair handles and legs, due to the use of 1D convolutions. On the other hand, by employing 32 decoders, our approach can both preserve smooth surface as well as capture thin structures, with results that best resemble the ground truth (GT).}
	\vspace{-12pt}
\end{figure}

\begin{figure*}[t]
\centering
\includegraphics[width=0.9\linewidth]{imgs/data.pdf}
\vspace{-8pt}
	\caption{\label{fig:data} \small
	\textbf{Image-to-shape reconstruction results from the test set.} The images shown are the input (black background), our results (32K points, rendered blue), and ground truth (rendered in light green). Qualitatively, our method is able to generate high-resolution point clouds faithfully capturing fine geometric details such as the chair legs, arms, airplane engines, monitor stands etc.}
	
\end{figure*}

In this section we present quantitative and qualitative results for single-view image-to-shape reconstruction.
Our training dataset consists of shapes from ShapeNet\cite{chang2015shapenet} and renderings from multiple views provided by \cite{choy20163d}.
There are a total of $50,000$ shapes spanning 13 categories, each shape rendered from $24$ random viewpoints using Blinn-Phong shading.
The training is done using all categories at once with 80\% of the total for training and 20\% for testing, which are splits suggested in \cite{choy20163d}.
This follows the same experimental setup as previous papers \cite{fan2016point, choy20163d, atlasnet, mrt18}.
However, unlike AtlasNet~\cite{atlasnet}, our network is trained in one stage, without the need to
train the decoder in an auto-encoder setting, before fine-tuning it with an image CNN in a second step. Our model is implemented in Python 2.7 using PyTorch and experiments are performed on TitanX GPUs.
We used Adam optimizer~\cite{kingma2014adam} with learning rate of $10^{-3}$, $\beta_1=0.9$, $\beta_2=0.99$
and without weight decay. The model is trained for 40 epochs and the learning rate is divided by 2 every 5 epochs.

\paragraph{Comparisons to state-of-the-art.} We have compared our approach with AtlasNet~\cite{atlasnet} and MRTNet~\cite{mrt18}.
For both of those methods, we used models provided by the authors and Chamfer distance
(Equation~\ref{eq:chamfer}) as evaluation metric.
All models are centered around center of gravity and scaled such that the point furthest away from the origin has distance 1 to the origin.
For a fair comparison, we use 4K points for evaluation across all methods.
Specifically, for our method (32 decoders) and AtlasNet, we select 4K points from the output point cloud uniformly at random; MRTNet already generates exactly 4K points, so no sampling is needed.
The evaluation results are presented in Table~\ref{tab:svr}.
Compared to MRTNet, our model performs better in 12 out of 13 categories. Compared to AtlasNet, our method is better or ties (the firearm category) in 7 out of 13 categories.
Overall our approach outperforms AtlasNet in per-category mean by 0.21, a relative improvement of 4.4\%. Also note that our model outperforms AtlasNet mainly in categories with
a large number of examples (tables, cars, airplanes, chairs). As a result, if average over instances, our method has a per-instance mean of 4.0, vs. 4.38 by AtlasNet -- a relatively improvement of  8.7\%.

\begin{table*}[t!]
\centering
{
\small
  \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|c|c|c||c}
   &  pla. &  ben. &  cab. &  car &  cha. &  mon. &  lam. &  spe. &  fir. &  cou. &  tab. &  cel. &  wat. &  \textbf{mean} \\
  \hline
 AtlasNet~\cite{atlasnet} &
2.17 &
\textbf{3.39} &
\textbf{3.93} &
3.40 &
4.56 &
\textbf{5.05} &
12.24 &
8.79 &
\textbf{2.15} &
\textbf{4.58} &
4.15 &
\textbf{3.25} &
3.93 &
4.74\\
 
 MRTNet~\cite{mrt18} &
2.25 &
3.68 &
4.73 &
\textbf{2.55} &
4.06 &
6.07 &
11.15 &
8.84 &
2.25 &
4.98 &
4.45 &
3.72 &
3.64 &
4.80\\



Ours (32 dec.)&
\textbf{2.06} &
3.40 &
4.46 &
2.60 &
\textbf{3.76} &
5.94 &
\textbf{10.66} &
\textbf{8.38} &
\textbf{2.15} &
4.64 &
\textbf{3.96} &
3.45 &
\textbf{3.40} &
\textbf{4.53} \\
  \end{tabular}
  }
\vspace{-4pt}
\caption{\small \textbf{Quantitative results for single-view image-to-shape reconstruction.} The table reports Chamfer distance metric (scaled by $10^3$) computed per category, and the mean of all categories.
For each method 4K points were used to compute the distance. %
  }
  \label{tab:svr}
\end{table*}

\paragraph{Ablation studies.} Table~\ref{tab:alt} shows a quantitative comparison between a few architectural variations.
We start by analyzing a variation of our network that generates the same number of points (using a single decoder) as MRTNet (4K points) and the same image encoder (vgg-16).
The performance of this variation is 0.05 worse than MRTNet, but it has an order of magnitude less parameters than MRTNet.
Another variation is to still use a single decoder but generate a higher-resolution point cloud (16K points).
This variation results in improved Chamfer distance, by 0.1, than the first variation, indicating that the increased resolution does improve reconstruction accuracy. Again, even when the number of generated points is higher than 4K, our evaluation is done by randomly selecting 4K points, for fair comparison. The last row in the table is our default setting (32 decoders outputting a total of 32K points). 
The number of network parameters are reported in Table~\ref{tab:param}. Even though the number of points our network generates is 8 times that of MRTNet, its size is only about 1/6 of MRTNet, since our network does not need to represent multiple resolutions at each layer. Compared to AtlasNet, our network is about 1/3 of its size, due to the efficiency of using a fully convolutional architecture. Despite using a much smaller number of parameters, our network outperforms MRTNet (in terms of Chamfer distance metric) by 0.27, and AtlasNet by 0.21.


\begin{table}
\centering
{
\begin{tabular}{|l|c|c|}
    \hline
    Architecture &  mean/cat. & mean/inst. \\
    \hline
    MRTNet & 4.80 & 4.26 \\
    1 dec./vgg16/4k & 4.85 & 4.30\\
    1 dec./res18/16k & 4.75 & 4.22\\
    32 dec./res18/32k & \textbf{4.53} & \textbf{4.00}\\
    \hline
\end{tabular}
}
\vspace{-4pt}
\caption{\label{tab:alt} \small
    \textbf{Architecture variations and evaluation results.} The table reports per-category mean and per-instance mean for MRTNet, and three variations of our methods: single decoder with 4K output points, 16K output points, and 32 decoders with 32 output points. For all cases, the Chamfer distance is calculated using 4K sample points, and results are scaled by $10^3$.
}
\end{table}

\begin{table}
\centering
{
\begin{tabular}{|l|c|}
    \hline
    Method &  \#parameters \\
    \hline
    AtlasNet & 42.6M \\
    MRTNet & 81.6M \\
    \hline 
    Ours (1 dec.) & 2.49M \\
    Ours (1 residual dec.) & 5.79M \\
    Ours (32 dec.) & 14.5M  \\
    \hline
\end{tabular}
}
\vspace{-4pt}
\caption{\label{tab:param} \small
    \textbf{Comparing the \# of network parameters.}
}
\end{table}

\paragraph{Qualitative Results.} Figure~\ref{fig:data} shows image-to-shape reconstruction results for images from the test dataset. Overall our method is able to accurately capture fine geometric details such as the chair legs, arms, airplane engines, monitor stands etc. The number of points (32K) is considerably higher than previous work (e.g. 1K by~\cite{fan2016point} and 4K by~\cite{mrt18}). Some specific shapes, such as lamps and jet fighters, present significant challenges for the network as the input images do not contain all the visual details. Nonetheless our method is able to produce a reasonable approximation.


\paragraph{Test on real images.} The test set images are synthetically rendered and as such they look similar to the training images. To evaluate our method on real images we use photos downloaded from the Internet, as shown in~\cite{mrt18}. They are processed by removing the background so only the foreground object remains. Figure~\ref{fig:toy} shows the results. The top row in the figure shows furniture objects, which demonstrate that even though the network is trained using synthetic images rendered with artificial lighting and materials, the model is able to generalize well to real shading, lighting, and materials. The second row shows additional objects where the shading is considerably different from training images. In particular, the last image (desktop computer) is in a category that the training has never seen. Nonetheless the reconstructed shape is reasonable.



\begin{figure*}[t]
\centering
\includegraphics[width=0.9\linewidth]{imgs/furniture.pdf}
\includegraphics[width=0.9\linewidth]{imgs/toys.pdf}
	\caption{\label{fig:toy} \small
	\textbf{Image-to-shape reconstruction results on Internet photos.} We test our method on real photos downloaded from the Internet and the results are rendered in blue. 
    The test images here are considerably different from the training set. Our method achieves reasonable results with accurate geometric details. The last image (computer) represents a category that has not been seen during training.
    }
\end{figure*}


\paragraph{Shape correspondence.} Once trained, our network learns to generate shapes with corresponding structures.
We demonstrate this with the following experiment.
First, we randomly select a point cloud generated by our network and call it a reference shape.
Then, we assign every point in the reference shape a color, where the hue is computed based on the point's distance to the center of gravity of the object.
Then this color assignment is propagated to the other point clouds, such that a point at index $(i,j)$ in the output tensor is assigned the same color as the point on the reference shape at the same index.
The resulting colorized point clouds are shown in Figure~\ref{fig:corresp}. Similar color indicates similar index range in the output tensor.
Note that even though the network is not trained explicitly with point correspondences as
supervisory signal, it learns to generate corresponding parts in the same
regions of the output tensor, as can be seen around
the tips of the chairs' arms,  legs and  seats.

\begin{figure*}[h!]
\centering
\includegraphics[width=0.8\linewidth]{imgs/corresp.pdf}
	\caption{\label{fig:corresp} \small
	\textbf{Visualizing Shape Correspondences.}
	Our network learns approximate shape correspondences even though the training is not supervised with such information. The shapes shown here are generated by 32 decoders.
	}
\end{figure*}

==> symbols.tex <==
\def\point{P}
\def\matrix{P}
\def\npoints{N}
\def\nshapes{S}
\def\nbasis{B}
\def\depth{D}
\def\scale{k}
\def\encoding{\mathbf{z}}
\newcommand{\para }[1]{\medskip \noindent {\bf #1}}
\def\mrtnet{MRTNet\xspace}
\def\mrvae{MR-VAE\xspace}
\def\kdtree{kd-tree\xspace}
\def\eg{\emph{e.g.}\xspace}
\def\ie{\emph{i.e.}\xspace}

